Parallel-in-time integration of the shallow water equations on the rotating sphere using Parareal and MGRIT

Despite the growing interest in parallel-in-time methods as an approach to accelerate numerical simulations in atmospheric modelling, improving their stability and convergence remains a substantial challenge for their application to operational models. In this work, we study the temporal parallelization of the shallow water equations on the rotating sphere combined with time-stepping schemes commonly used in atmospheric modelling due to their stability properties, namely an Eulerian implicit-explicit (IMEX) method and a semi-Lagrangian semi-implicit method (SL-SI-SETTLS). The main goal is to investigate the performance of parallel-in-time methods, namely Parareal and Multigrid Reduction in Time (MGRIT), when these well-established schemes are used on the coarse discretization levels and provide insights on how they can be improved for better performance. We begin by performing an analytical stability study of Parareal and MGRIT applied to a linearized ordinary differential equation depending on the choice of a coarse scheme. Next, we perform numerical simulations of two standard tests to evaluate the stability, convergence and speedup provided by the parallel-in-time methods compared to a fine reference solution computed serially. We also conduct a detailed investigation on the influence of artificial viscosity and hyperviscosity approaches, applied on the coarse discretization levels, on the performance of the temporal parallelization. Both the analytical stability study and the numerical simulations indicate a poorer stability behaviour when SL-SI-SETTLS is used on the coarse levels, compared to the IMEX scheme. With the IMEX scheme, a better trade-off between convergence, stability and speedup compared to serial simulations can be obtained under proper parameters and artificial viscosity choices, opening the perspective of the potential competitiveness for realistic models.

==> numerical_tests/numerical_tests_pint.tex <==
\subsection{Parallel-in-time simulations}

\indent In all parallel-in-time simulations presented in this section, we fix the discretization in the finest level, with a relatively small time step size and large spectral discretization; for the coarse level(s), we consider various temporal and spectral discretization. We also vary the number of levels and the relaxation strategy adopted in MGRIT.

\subsection{Convergence study}

\subsubsection{Gaussian bump}

\indent In this first test case, the finest level in the PinT configuration is discretized with a spectral resolution $M_0 = 256$, time step size $\Dt_0 = 60$ and artificial viscosity coefficient $\nu_0 = 10^5$. The serial solution obtained under these configurations is called hereafter as \quotes{fine solution}, in opposition to the \quotes{reference solution} described above ($M_{\text{ref}} = 1024$, $\Dt_{\text{ref}} = 2$, $\nu_{\text{ref}} = 0$). We perform MGRIT simulations considering $\nlevels \in \{2,3\}$, with a coarsening factor $\cfactor \in \{2, 4\}$. The same spectral resolution is considered in all coarse levels, being set to $M_{\text{coarse}} \in \{51, 128\}$, which correspond respectively to $1/5$ and $1/2$ of the spectral resolution in the finest level. We also consider several relaxation strategies, with $\nrelax \in \{0,1,2\}$. We recall that MGRIT with $(\nlevels, \nrelax) = (2,0)$ is equivalent to Parareal.

\indent Figure \ref{fig:errors_params_mgrit} presents the evolution, along with iterations, of the relative spectral error between the parallel-in-time and the fine solution. The errors are shown for two chosen spectral resolutions, namely $\rnorm = 32$ and $\rnorm = 128$. We observe that only a few simulations are stable and able to converge, namely when the spectral resolution in the coarse levels, the number of levels, and/or the coarsening factor are sufficiently small; when this is not the case, the time step in the coarsest level are too significant and lead to unstable behaviors. With $\Mcoarse = 51$, all configurations can converge, more or less rapidly, at the beginning of the wavenumber spectrum ($\rnorm = 32$), except for the most aggressive configuration ($(\nlevels, \cfactor) = (3,4)$); when more modes are considered in the error analysis ($\rnorm = 128$), the simulations with $(\nlevels, \cfactor) = (2,4)$, which presents the fastest convergence with ($\rnorm = 32$), also starts to develop instabilities that compromise convergence. On the other hand, when a finer spectral resolution in the coarse levels is considered ($\Mcoarse = 128$), none of the MGRIT configurations is stable, even with $\rnorm = 32$. The less aggressive one ($(\nlevels, \cfactor) = (3,4)$) initially presents a converging behavior, but the error starts to increase after five iterations; under other configurations, the instabilities start to develop even sooner. Finally, in almost all configurations, we notice a small convergence improvement when the relaxation strategy is more expensive (\ie when $\nrelax$ increases). Still, the error and stability behaviors are essentially the same.

\begin{figure}[!htbp]
    \begin{subfigure}{.5\linewidth}
        \centering
        \includegraphics[scale=.45]{numerical_tests/figures/numerical_tests_pint/gaussian_bump/errors/error_fine_rnorm_32_runtime.xbraid_spatial_coarsening_51__.pdf}
        \caption{$M_{\text{coarse}} = 51$, $\rnorm = 32$}
    \end{subfigure}
    \begin{subfigure}{.5\linewidth}
        \centering
        \includegraphics[scale=.45]{numerical_tests/figures/numerical_tests_pint/gaussian_bump/errors/error_fine_rnorm_128_runtime.xbraid_spatial_coarsening_51__.pdf}
        \caption{$M_{\text{coarse}} = 51$, $\rnorm = 128$}
    \end{subfigure}
    \begin{subfigure}{.5\linewidth}
        \centering
        \includegraphics[scale=.45]{numerical_tests/figures/numerical_tests_pint/gaussian_bump/errors/error_fine_rnorm_32_runtime.xbraid_spatial_coarsening_128__.pdf}
        \caption{$M_{\text{coarse}} = 128$, $\rnorm = 32$}
    \end{subfigure}
    \begin{subfigure}{.5\linewidth}
        \centering
        \includegraphics[scale=.45]{numerical_tests/figures/numerical_tests_pint/gaussian_bump/errors/error_fine_rnorm_128_runtime.xbraid_spatial_coarsening_128__.pdf}
        \caption{$M_{\text{coarse}} = 128$, $\rnorm = 128$}
    \end{subfigure}
    \caption{Relative error $L_{\infty(\rnorm)}$ between the PinT and the fine solution along iterations, for $\rnorm = 32$ (left) and $\rnorm = 128$ (right); and $\Mcoarse = 51$ (top) and $\Mcoarse = 128$ (bottom). Simulations are identified by $(\nlevels, \cfactor, \nrelax)$. }
    \label{fig:errors_params_mgrit}
\end{figure}

\indent The same error plots, but computed \wrt the reference solution instead of the fine one, are presented in Figure \ref{fig:errors_params_mgrit_ref}. The convergence and stability behaviors are similar to those in Figure \ref{fig:errors_params_mgrit}, but naturally leads to larger errors since the MGRIT solution converges to the fine one. We observe that, in the best-performing simulations, the error relative to the reference solution decreases by factors no larger than 4 after ten iterations.
In contrast, decreases of almost two orders of magnitude are obtained  when the error is computed \wrt the fine solution.


\begin{figure}[!htbp]
    \begin{subfigure}{.5\linewidth}
        \centering
        \includegraphics[scale=.45]{numerical_tests/figures/numerical_tests_pint/gaussian_bump/errors/error_ref_rnorm_32_runtime.xbraid_spatial_coarsening_51__.pdf}
        \caption{$M_{\text{coarse}} = 51$, $\rnorm = 32$}
    \end{subfigure}
    \begin{subfigure}{.5\linewidth}
        \centering
        \includegraphics[scale=.45]{numerical_tests/figures/numerical_tests_pint/gaussian_bump/errors/error_ref_rnorm_128_runtime.xbraid_spatial_coarsening_51__.pdf}
        \caption{$M_{\text{coarse}} = 51$, $\rnorm = 128$}
    \end{subfigure}
    \begin{subfigure}{.5\linewidth}
        \centering
        \includegraphics[scale=.45]{numerical_tests/figures/numerical_tests_pint/gaussian_bump/errors/error_ref_rnorm_32_runtime.xbraid_spatial_coarsening_128__.pdf}
        \caption{$M_{\text{coarse}} = 128$, $\rnorm = 32$}
    \end{subfigure}
    \begin{subfigure}{.5\linewidth}
        \centering
        \includegraphics[scale=.45]{numerical_tests/figures/numerical_tests_pint/gaussian_bump/errors/error_ref_rnorm_128_runtime.xbraid_spatial_coarsening_128__.pdf}
        \caption{$M_{\text{coarse}} = 128$, $\rnorm = 128$}
    \end{subfigure}
    \caption{Relative error $L_{\infty(\rnorm)}$ between the PinT and the reference solution along iterations, for $\rnorm = 32$ (left) and $\rnorm = 128$ (right); and $\Mcoarse = 51$ (top) and $\Mcoarse = 128$ (bottom). Simulations are identified by $(\nlevels, \cfactor, \nrelax)$. }
    \label{fig:errors_params_mgrit_ref}
\end{figure}

\indent The obtained errors can be better understood by observing the relative difference between the PinT and the reference geopotential fields, which is illustrated in Figure \ref{fig:solution_params_mgrit} for two chosen configurations, namely $(\nlevels,\cfactor,\nrelax,\Mcoarse) = (2,4,2,128)$ and $(\nlevels,\cfactor,\nrelax,\Mcoarse) = (3,2,2,51)$, the former developing instabilities after a good convergence in the first five iterations, whereas the latter presents a monotonic convergence behavior. in the configuration $(\nlevels,\cfactor,\nrelax,\Mcoarse) = (2,4,2,128)$, the magnitude of the errors decrease from the initial to the fifth iteration (compare the color bar scales), but small oscillations develop in the entire spatial domain, which illustrates the converging behavior with $\rnorm = 32$ but already increasing error with $\rnorm = 128$ (see Figure \ref{fig:errors_params_mgrit}). After ten iterations, the instabilities lead to errors whose magnitudes are larger than the initial ones. On the other hand, in the configuration $(\nlevels,\cfactor,\nrelax,\Mcoarse) = (3,2,2,51)$, the error magnitude decreases along iterations; in the fifth-one, much smaller oscillations can be observed, and they visually almost completely vanish after ten iterations.


\begin{figure}[!htbp]
    \begin{subfigure}{.5\linewidth}
        \includegraphics[scale=.35]{numerical_tests/figures/numerical_tests_pint/gaussian_bump/solution/nlevels2_mc4_nrelax2_coarsening128/plot_prog_phi_t00000000028.44444444_iter000_map_full_comparison_fine_diff.pdf}
        \caption{$(\nlevels,\cfactor,\nrelax,\Mcoarse) = (2,2,2,128)$, iteration 0}
        \vspace*{10pt}
    \end{subfigure}
    \begin{subfigure}{.5\linewidth}
        \includegraphics[scale=.35]{numerical_tests/figures/numerical_tests_pint/gaussian_bump/solution/nlevels3_mc2_nrelax2_coarsening51/plot_prog_phi_t00000000028.44444444_iter000_map_full_comparison_fine_diff.pdf}        \caption{$(\nlevels,\cfactor,\nrelax,\Mcoarse) = (3,2,2,51)$, iteration 0}
        \vspace*{10pt}
    \end{subfigure}
    \begin{subfigure}{.5\linewidth}
        \includegraphics[scale=.35]{numerical_tests/figures/numerical_tests_pint/gaussian_bump/solution/nlevels2_mc4_nrelax2_coarsening128/plot_prog_phi_t00000000028.44444444_iter005_map_full_comparison_fine_diff.pdf}
        \caption{$(\nlevels,\cfactor,\nrelax,\Mcoarse) = (2,2,2,128)$, iteration 5}
        \vspace*{10pt}
    \end{subfigure}
    \begin{subfigure}{.5\linewidth}
        \includegraphics[scale=.35]{numerical_tests/figures/numerical_tests_pint/gaussian_bump/solution/nlevels3_mc2_nrelax2_coarsening51/plot_prog_phi_t00000000028.44444444_iter005_map_full_comparison_fine_diff.pdf}
        \caption{$(\nlevels,\cfactor,\nrelax,\Mcoarse) = (3,2,2,51)$, iteration 5}
        \vspace*{10pt}
    \end{subfigure}
    \begin{subfigure}{.5\linewidth}
        \includegraphics[scale=.35]{numerical_tests/figures/numerical_tests_pint/gaussian_bump/solution/nlevels2_mc4_nrelax2_coarsening128/plot_prog_phi_t00000000028.44444444_iter010_map_full_comparison_fine_diff.pdf}
        \caption{$(\nlevels,\cfactor,\nrelax,\Mcoarse) = (2,2,2,128)$, iteration 10}
        \vspace*{10pt}
    \end{subfigure}
    \begin{subfigure}{.5\linewidth}
        \includegraphics[scale=.35]{numerical_tests/figures/numerical_tests_pint/gaussian_bump/solution/nlevels3_mc2_nrelax2_coarsening51/plot_prog_phi_t00000000028.44444444_iter010_map_full_comparison_fine_diff.pdf}
        \caption{$(\nlevels,\cfactor,\nrelax,\Mcoarse) = (3,2,2,51)$, iteration 10}
        \vspace*{10pt}
    \end{subfigure}
        \caption{Relative difference between the parallel-in-time and reference (fine) geopotential field at $t = T$, under MGRIT configurations $(\nlevels,\cfactor,\nrelax,\Mcoarse) = (2,2,2,128)$ (left) and $(\nlevels,\cfactor,\nrelax,\Mcoarse) = (3,2,2,51)$ (right) at iterations 0, 5 and 10 (respectively first, second and third rows).}
        \label{fig:solution_params_mgrit}
\end{figure}

\indent The stability and convergence behaviors of the two simulations presented in Figure \ref{fig:solution_params_mgrit} are also illustrated in Figure \ref{fig:gaussian_bump_spectrum}, in which we compare the kinetic energy (KE) spectrum at $t = T$ in given iterations with those corresponding to the fine and reference solutions. For a triangular spectral truncation, the KE spectrum is defined by \cite{koshyk_hamilton:2001}

\begin{equation*}
    E(n, t) = \frac{1}{4} \frac{a^2}{n(n+1)} \sum_{m = -n}^n\left( |\xi_{m,n}(t)|^2 + |\delta_{m,n}(t)|^2 \right)
\end{equation*}

\noindent where $\xi_{m,n}(t)$ and $\delta_{m,n}(t)$ are the spherical harmonics coefficients of the vorticity and divergence, respectively. In Figure \ref{fig:gaussian_bump_spectrum}, we present the spectrum in the function of the wavelength $\mc{L}_n := 2\pi a / n$. Notice that the spectra of the fine and MGRIT solutions cover smaller wavelength ranges than the reference solution due to the adopted truncations ($M_0 = 256$ and $M_{\text{ref}} = 1024$); also, the fine solution has a stronger decay of larger wavenumbers (smaller wavelengths) than the reference one due to the adopted viscosity coefficients ($\nu_0 = 10^5$ and $\nu_{\text{ref}} = 0$). Concerning the MGRIT simulations, the unstable behavior using $(\nlevels,\cfactor,\nrelax,\Mcoarse) = (2,2,2,128)$ is clear in the spectrum, with over-amplifications of large wavenumbers along iterations. On the other hand, the spectrum of the simulation using $(\nlevels,\cfactor,\nrelax,\Mcoarse) = (3,2,2,51)$ remains below the fine one but slowly converging to it, indicating a more difficult convergence of large wavenumber modes. 

\begin{figure}
    \centering
    \includegraphics[scale=.5]{numerical_tests/figures/numerical_tests_pint/gaussian_bump/spectrum/spec.pdf}
    \caption{Kinetic energy spectra of the fine (green line), reference (red line) and MGRIT solutions using $(\nlevels,\cfactor,\nrelax,\Mcoarse) = (3,2,2,51)$ (blue lines) and $(\nlevels,\cfactor,\nrelax,\Mcoarse) = (2,2,2,128)$ (orange lines). The MGRIT spectra are presented for iterations 0, 5, and 10.} 
    \label{fig:gaussian_bump_spectrum}
\end{figure}


\subsubsection{Unstable jet}


\subsection{Performance study}

\subsection{Influence of artificial diffusion}

\indent In all simulations presented above, an artificial second-order diffusion approach was considered, as described in Section \ref{subsec:governing_equations}, with the same viscosity coefficient ($\nu = 10^5$) being applied to all MGRIT discretization levels. In the following paragraphs, we propose a finer study on the influence of artificial viscosity on the stability and convergence of temporal parallelization. For each test case, we select an MGRIT configuration and run simulations considering various (and possibly different) viscosity values at each level.

\subsubsection{Gaussian bump}

\indent For the Gaussian bump test case, we perform this study considering the configuration $(\nlevels, \cfactor, \nrelax, \Mcoarse) = (2, 2, 0, 128)$. As shown in Figure \ref{fig:errors_params_mgrit}, it results in an initial converging behavior but diverges after a few iterations at low and high regions of the wavenumber spectrum. We perform simulations with the viscosity coefficient of the fine ($\nu_0$) and the coarse ($\nu_{\text{coarse}}$) levels taking value in $\{0, 1o^4, 10^5, 10^6\}$. The evolution of the errors along iterations, \wrt the fine solution, is presented in Figure \ref{fig:viscosity_erros_gaussian_bump_2}. For the sake of readability, the curves are separated in two plots, respectively, with $\nu_0 \in \{0, 10^4\}$ and $\nu_0 \in \{10^5, 10^6\}$.

\indent We observe from these results that, for relatively low diffusion coefficients in the fine level ($\nu_0 = 0$ and $\nu_0 = 10^4$), the convergence and stability are determined mainly by the diffusion coefficient in the coarse level, being little influenced by $\nu_0$ itself. Choosing $\nu_{\text{coarse}}$ large enough ensures convergence and stability, mainly \wrt the errors measured at large wavenumbers; otherwise, instabilities begin to be observed after a few iterations. The influence of $\nu_0$ is more remarkable when large values of it are compared ($\nu_0 = 10^5$ and $\nu_0 = 10^6$): simulations seem more stable, having a monotonic decreasing error or a later diverging behavior, when $\nu_0$ is smaller. The only exception is when both fine and coarse levels have a large diffusion coefficient ($\nu_0 = \nu_{\text{coarse}} = 10^6$), in which case it is observed a fast convergence towards errors of several orders of magnitude smaller than those under other viscosity coefficient values.


\begin{figure}[!htbp]
    \begin{subfigure}{.5\linewidth}
        \centering
        \includegraphics[scale=.45]{numerical_tests/figures/numerical_tests_pint/gaussian_bump/viscosity/errors/nlevels2_mc2_nrelax0_coarsening128/visc_0_1e4/error_fine_rnorm_32_runtime.xbraid_max_levels_2__runtime.xbraid_cfactor_2__runtime.xbraid_nrelax_0__runtime.xbraid_spatial_coarsening_128__.pdf}
        \caption{$\nu_0 = 0$ and $\nu_0 = 10^4$; $\rnorm = 32$}
    \end{subfigure}
    \begin{subfigure}{.5\linewidth}
        \centering
        \includegraphics[scale=.45]{numerical_tests/figures/numerical_tests_pint/gaussian_bump/viscosity/errors/nlevels2_mc2_nrelax0_coarsening128/visc_0_1e4/error_fine_rnorm_128_runtime.xbraid_max_levels_2__runtime.xbraid_cfactor_2__runtime.xbraid_nrelax_0__runtime.xbraid_spatial_coarsening_128__.pdf}
        \caption{$\nu_0 = 0$ and $\nu_0 = 10^4$; $\rnorm = 128$}
    \end{subfigure}
    \begin{subfigure}{.5\linewidth}
        \centering
        \includegraphics[scale=.45]{numerical_tests/figures/numerical_tests_pint/gaussian_bump/viscosity/errors/nlevels2_mc2_nrelax0_coarsening128/visc_1e5_1e6/error_fine_rnorm_32_runtime.xbraid_max_levels_2__runtime.xbraid_cfactor_2__runtime.xbraid_nrelax_0__runtime.xbraid_spatial_coarsening_128__.pdf}
        \caption{$\nu_0 = 10^5$ and $\nu_0 = 10^6$; $\rnorm = 32$}
    \end{subfigure}
    \begin{subfigure}{.5\linewidth}
        \centering
        \includegraphics[scale=.45]{numerical_tests/figures/numerical_tests_pint/gaussian_bump/viscosity/errors/nlevels2_mc2_nrelax0_coarsening128/visc_1e5_1e6/error_fine_rnorm_128_runtime.xbraid_max_levels_2__runtime.xbraid_cfactor_2__runtime.xbraid_nrelax_0__runtime.xbraid_spatial_coarsening_128__.pdf}
        \caption{$\nu_0 = 10^4$ and $\nu_0 = 10^6$; $\rnorm = 128$}
    \end{subfigure}
    \caption{Relative error $L_{\infty(\rnorm)}$ between the PinT and the fine solution along iterations, for $(\nlevels, \cfactor, \nrelax, \Mcoarse) = (2, 4, 0, 128)$. Left and right columns: $\rnorm = 32$ and $\rnorm = 128$, respectively. Top and bottom rows: $\nu \in \{0, 10^4\}$ and $\nu \in \{10^5, 10^6\}$, respectively. Simulations are identified by $(\nu_0, \nu_{\text{coarse}})$.}
    \label{fig:viscosity_erros_gaussian_bump_2}
\end{figure}

\indent These results, however, should be analyzed very carefully. Indeed, the errors presented in Figure \ref{fig:viscosity_erros_gaussian_bump_2} refer to the fine solution, which is the solution MGRIT converges to (instead of the \quotes{true} solution of the problem). Therefore, the observed convergence under $\nu_0 = 10^6$ may be due to a possible overdamping of high wavenumbers: the poor convergence with $\nu_{\text{coarse}} < 10^6$ is due to an introduction of finer modes from the coarse to fine level, whereas the fast convergence with $\nu_{\text{coarse}} = 10^6$ reflects the fact that both fine and coarse levels resolve only smaller spatial features of the solution, which is known to be an easier task in the context of temporal parallelization. These remarks can be better understood by observing the errors \wrt the reference solution computed with a very small time size and a much finer spectral discretization (Figure \ref{fig:viscosity_erros_gaussian_bump_2_ref}): while the error evolution is essentially the same as in Figure \ref{fig:viscosity_erros_gaussian_bump_2} for $\nu_0 < 10^6$ (obviously converging to larger errors), the solution for $\nu_0 = 10^6$ has no error decrease at all (and even an error increase from the initial iteration for some configurations), indicating that the fine solution is not a good representation of the solution of the problem due to the application of a too large artificial viscosity.

\begin{figure}[!htbp]
    \begin{subfigure}{.5\linewidth}
        \centering
        \includegraphics[scale=.45]{numerical_tests/figures/numerical_tests_pint/gaussian_bump/viscosity/errors/nlevels2_mc2_nrelax0_coarsening128/visc_0_1e4/error_ref_rnorm_32_runtime.xbraid_max_levels_2__runtime.xbraid_cfactor_2__runtime.xbraid_nrelax_0__runtime.xbraid_spatial_coarsening_128__.pdf}
        \caption{$\nu_0 = 0$ and $\nu_0 = 10^4$; $\rnorm = 32$}
    \end{subfigure}
    \begin{subfigure}{.5\linewidth}
        \centering
        \includegraphics[scale=.45]{numerical_tests/figures/numerical_tests_pint/gaussian_bump/viscosity/errors/nlevels2_mc2_nrelax0_coarsening128/visc_0_1e4/error_ref_rnorm_128_runtime.xbraid_max_levels_2__runtime.xbraid_cfactor_2__runtime.xbraid_nrelax_0__runtime.xbraid_spatial_coarsening_128__.pdf}
        \caption{$\nu_0 = 0$ and $\nu_0 = 10^4$; $\rnorm = 128$}
    \end{subfigure}
    \begin{subfigure}{.5\linewidth}
        \centering
        \includegraphics[scale=.45]{numerical_tests/figures/numerical_tests_pint/gaussian_bump/viscosity/errors/nlevels2_mc2_nrelax0_coarsening128/visc_1e5_1e6/error_ref_rnorm_32_runtime.xbraid_max_levels_2__runtime.xbraid_cfactor_2__runtime.xbraid_nrelax_0__runtime.xbraid_spatial_coarsening_128__.pdf}
        \caption{$\nu_0 = 10^5$ and $\nu_0 = 10^6$; $\rnorm = 32$}
    \end{subfigure}
    \begin{subfigure}{.5\linewidth}
        \centering
        \includegraphics[scale=.45]{numerical_tests/figures/numerical_tests_pint/gaussian_bump/viscosity/errors/nlevels2_mc2_nrelax0_coarsening128/visc_1e5_1e6/error_ref_rnorm_128_runtime.xbraid_max_levels_2__runtime.xbraid_cfactor_2__runtime.xbraid_nrelax_0__runtime.xbraid_spatial_coarsening_128__.pdf}
        \caption{$\nu_0 = 10^4$ and $\nu_0 = 10^6$; $\rnorm = 128$}
    \end{subfigure}
    \caption{Relative error $L_{\infty(\rnorm)}$ between the PinT and the reference solution along iterations, for $(\nlevels, \cfactor, \nrelax, \Mcoarse) = (2, 4, 0, 128)$. Left and right columns: $\rnorm = 32$ and $\rnorm = 128$, respectively. Top and bottom rows: $\nu \in \{0, 10^4\}$ and $\nu \in \{10^5, 10^6\}$, respectively. Simulations are identified by $(\nu_0, \nu_{\text{coarse}})$.}
    \label{fig:viscosity_erros_gaussian_bump_2_ref}
\end{figure}

\indent Figure \ref{fig:viscosity_solution_gaussian_bump} illustrates the solution obtained with different viscosity values, namely $(\nu_0,\nu_{\text{coarse}}) = (10^6,10^5)$ and $(\nu_0,\nu_{\text{coarse}}) = (10^6,10^6)$, focusing on the region of the spatial domain containing the largest gradients of the geopotential field at $t = T$. Under both viscosity configurations, strong damping of fine spatial features of the solution is observed, and notably, the peak in the geopotential field around the longitude $\lambda = 180^{\circ}$ is no longer observed. With $(\nu_0,\nu_{\text{coarse}}) = (10^6,10^5)$, the absence of viscosity in the coarse level introduces energy in the fine wavenumbers, leading to visible instabilities; with $(\nu_0,\nu_{\text{coarse}}) = (10^6,10^6)$, the solution's profile remains too smoothed due to the large viscosity coefficient in the coarse level, explaining the fast convergence behavior towards the fine solution (Figure \ref{fig:viscosity_erros_gaussian_bump_2}) and the lack of convergence towards the reference one (Figure \ref{fig:viscosity_erros_gaussian_bump_2_ref}).  


\begin{figure}[!htbp] 
    \begin{subfigure}{\linewidth}
        \centering
        \includegraphics[scale=.4]{numerical_tests/figures/reference_solution/gaussian_bump/plots/plot_prog_phi_t00000000028.44444444_map_zoom_gaussian_bump.pdf}
        \caption{Reference solution}
        \vspace*{10pt}
    \end{subfigure}
    \begin{subfigure}{.5\linewidth}
        \includegraphics[scale=.35]{numerical_tests/figures/numerical_tests_pint/gaussian_bump/viscosity/solution/nlevels2_mc2_nrelax0_coarsening128_visc1e5/plot_prog_phi_t00000000028.44444444_iter000.pdf}
        \caption{$(\nu_0, \nu_{\text{coarse}}) = (10^6, 10^5)$, iteration 0}
        \vspace*{10pt}
    \end{subfigure}
    \begin{subfigure}{.5\linewidth}
        \includegraphics[scale=.35]{numerical_tests/figures/numerical_tests_pint/gaussian_bump/viscosity/solution/nlevels2_mc2_nrelax0_coarsening128_visc1e5/plot_prog_phi_t00000000028.44444444_iter005.pdf}
        \caption{$(\nu_0, \nu_{\text{coarse}}) = (10^6, 10^5)$, iteration 5}
        \vspace*{10pt}
    \end{subfigure}
    \begin{subfigure}{.5\linewidth}
        \includegraphics[scale=.35]{numerical_tests/figures/numerical_tests_pint/gaussian_bump/viscosity/solution/nlevels2_mc2_nrelax0_coarsening128_visc1e6/plot_prog_phi_t00000000028.44444444_iter000.pdf}
        \caption{$(\nu_0, \nu_{\text{coarse}}) = (10^6, 10^6)$, iteration 0}
    \end{subfigure}
    \begin{subfigure}{.5\linewidth}
        \includegraphics[scale=.35]{numerical_tests/figures/numerical_tests_pint/gaussian_bump/viscosity/solution/nlevels2_mc2_nrelax0_coarsening128_visc1e6/plot_prog_phi_t00000000028.44444444_iter005.pdf}
        \caption{$(\nu_0, \nu_{\text{coarse}}) = (10^6, 10^6)$, iteration 5}
    \end{subfigure}
    \caption{Comparison between the reference solution (top) and PinT solutions obtained with $(\nlevels,\cfactor,\nrelax,\Mcoarse) = (2,2,0,128)$ at $t = T$ after the initial (left column) and fifth iterations (right column). Second and third rows: $(\nu_0,\nu_{\text{coarse}}) = (10^6,10^5)$ and $(\nu_0,\nu_{\text{coarse}}) = (10^6,10^6)$, respectively. Zoom in $(\lambda, \theta) \in [130^{\circ},230^{\circ}] \times [-75^{\circ}, 25^{\circ}]$}
    \label{fig:viscosity_solution_gaussian_bump}
\end{figure}

\indent The behavior of the simulations using the overdamped fine solution ($\nu_0 = 10^6$) in terms of the kinetic energy spectrum is illustrated in Figure \ref{fig:gaussian_bump_spectrum_viscosity} for all tested values of $\nu_{\text{coarse}}$ under the MGRIT configuration $(\nlevels,\cfactor,\nrelax,\Mcoarse) = (2,2,0,128)$. We observe that the largest wavenumbers in the fine solution are highly damped \wrt the reference one. Among all viscosity coefficients in the coarse level, only the simulation with $\nu_{\text{coarse}} = \nu_0 = 10^6$ starts at the initial iterations with its spectrum below the fine one, being able to provide a very good approximation to it after five iterations. For all other values of $\nu_{\text{coarse}}$, the spectrum starts above the fine one, and after five iterations almost the entire spectrum, including small and medium wavenumbers, is largely amplified.


\begin{figure}
    \centering
    \includegraphics[scale=.5]{numerical_tests/figures/numerical_tests_pint/gaussian_bump/viscosity/spectrum/spec.pdf}
    \caption{Kinetic energy spectra of the fine, reference, and MGRIT solutions using $(\nlevels,\cfactor,\nrelax,\Mcoarse) = (2,2,0,128)$, $\nu_0 = 10^6$ and various values of $\nu_{\text{coarse}}$.} 
    \label{fig:gaussian_bump_spectrum_viscosity}
\end{figure}
